ExecHMR: Transition-Aware Recovery of Robot-Executable Human Motion with Bidirectional Alignment

Human motion recovery (HMR) from monocular video enables humanoid robot imitation, yet existing methods prioritize pose accuracy without explicitly modeling the transition dynamics required for reliable robot execution. Recent post-hoc fine-tuning with simulation-based tracking feedback treats recovery fidelity and executability as separate objectives, although human motion and robot action describe the same underlying aligned movement. We introduce ExecHMR, which jointly models human motion recovery and robot action prediction in a single training stage through inter-frame transition reasoning. ExecHMR uses a shared temporal Transformer with human reconstruction and temporal action branches, learning inter-frame transition dynamics for reliable execution from controller commands recorded in closed-loop simulation. To unify the two branches around this shared movement, bidirectional kinematic alignment matches label-relative residuals in a common kinematic space and alternates teacher roles, enabling mutual guidance while preserving single-pass inference. On test videos from 3DPW, EMDB and RICH, ExecHMR achieves 86.0% execution success, compared with 79.7% for GENMO and 76.3% for FlowHMR, leading all six baselines with the largest gains on fast motions. It also achieves the lowest camera-space errors on 3DPW and EMDB-1 among compared methods, and we demonstrate deployment on a physical humanoid.

==> figures/align/align_pts.tex <==
% generated by paper_sa120/scripts/method_align_compose.py (frame 130, body right_wrist); normalised image coordinates, y up%
\def\baHumAspect{0.3234}%
\def\baHumZa{0.1196,0.5226}%
\def\baHumZb{0.8555,0.7606}%
\def\baHumZL{0.4294,0.2824}%
\def\baHumZP{0.4048,0.7180}%
\def\baHumZT{0.5945,0.3848}%
\def\baRobAspect{0.5159}%
\def\baRobZa{-0.0056,0.5965}%
\def\baRobZb{0.5712,0.8941}%
\def\baRobZL{0.6090,0.2825}%
\def\baRobZP{0.2953,0.4137}%
\def\baRobZT{0.7036,0.7169}%


==> figures/overview/align_pts.tex <==
% generated by paper_sa120/scripts/align_assets_compose.py: 14 compared bodies (hips, knees, ankles, waist,
% neck, shoulders, elbows, wrists; left before right) in coordinates normalised to align_{human,robot}.png
\def\alignHumanPts{0.531/0.494, 0.348/0.485, 0.620/0.277, 0.267/0.280, 0.661/0.097, 0.418/0.260, 0.420/0.607, 0.350/0.803, 0.617/0.793, 0.142/0.778, 0.885/0.688, 0.118/0.640, 0.628/0.637, 0.152/0.578}
\def\alignRobotPts{0.620/0.512, 0.322/0.525, 0.584/0.289, 0.235/0.308, 0.607/0.086, 0.351/0.206, 0.477/0.580, 0.470/0.833, 0.647/0.786, 0.311/0.791, 0.931/0.667, 0.160/0.673, 0.676/0.648, 0.206/0.625}
\def\alignHumanAspect{2.8080}
\def\alignRobotAspect{2.3745}
\def\alignHumanPx{702}
\def\alignRobotPx{653}


==> figures/real_supp_tikz.tex <==
% Supplementary real-robot deployments in the format of Fig. 6 (figures/real_robot.tex): per instant, the input frame,
% the camera-frame mesh of ExecHMR (s500k) over it (same crop) and the LimX Luna recording at the aligned instant (one
% constant offset per video from ViTPose limb directions). Tiles and pose similarities from
% paper_sa120/scripts/real3_assets.py (data/real3/fidelity_<clip>.json).
\definecolor{rrOurs}{RGB}{40,92,186}
% #1 clip letter (tiles figures/real_supp/<clip>_{in,mesh,robot}<n>.jpg), #2 {column/seconds/similarity,...}
\newcommand{\realsupp}[2]{%
\resizebox{\textwidth}{!}{%
\begin{tikzpicture}[x=1pt,y=1pt,font=\scriptsize]
\def\tw{48}\def\th{72.33}\def\tg{1.6}\def\rg{1.6}\def\bw{25}% tile (aspect 0.664 as Fig. 6), gaps, bar
\def\tile##1##2##3{%
  \begin{scope}
    \clip[rounded corners=1.5pt] (##1,##2) rectangle ++(\tw,\th);
    \node[anchor=south west,inner sep=0pt] at (##1,##2) {\includegraphics[width=\tw pt,height=\th pt]{##3}};
  \end{scope}
  \draw[rounded corners=1.5pt,draw=black!25,line width=0.3pt] (##1,##2) rectangle ++(\tw,\th);}%
\pgfmathsetmacro\ym{\th+\rg}\pgfmathsetmacro\yv{2*(\th+\rg)}%
\foreach \c/\t/\s in {#2}{
  \pgfmathsetmacro\tx{(\c-1)*(\tw+\tg)}
  \tile{\tx}{\yv}{figures/real_supp/#1_in\c.jpg}
  \tile{\tx}{\ym}{figures/real_supp/#1_mesh\c.jpg}
  \tile{\tx}{0}{figures/real_supp/#1_robot\c.jpg}
  \node[anchor=north west,inner sep=1pt,fill=black,fill opacity=0.55,text opacity=1,text=white,rounded corners=1pt,
        font=\fontsize{6.4}{7}\selectfont\bfseries] at (\tx+1.5,\yv+\th-1.5) {\t\,s};
  \fill[black!10,rounded corners=1.2pt] (\tx+1.5,-6.6) rectangle ++(\bw,3);
  \fill[rrOurs,rounded corners=1.2pt] (\tx+1.5,-6.6) rectangle ++(\bw*\s,3);
  \node[anchor=east,inner sep=0pt,text=rrOurs,font=\fontsize{7}{7.6}\selectfont\bfseries] at (\tx+\tw-0.8,-5.1) {\s};}
\end{tikzpicture}}}


==> figures/supp_cases_tikz.tex <==
% Supplementary cases in the format of the teaser (Fig. 1, figures/teaser_tikz.tex): per clip, video frames with the
% camera-frame mesh of ExecHMR (s500k), GENMO -> robot and ExecHMR robot mode, each robot frame rendered from the video
% camera's viewpoint relative to the person (paper_sa120/scripts/supp_cases_assets.sh; tiles: ffmpeg scale=360:480).
\definecolor{tsOurs}{RGB}{40,92,186}
\definecolor{tsBase}{RGB}{92,92,92}
\definecolor{tsFall}{RGB}{204,45,38}
\definecolor{tsOk}{RGB}{34,139,62}
% #1 tile prefix, #2 time axis {column/seconds,...}, #3 time at which the GENMO robot fell (last column shows it down)
\newcommand{\suppcase}[3]{%
\resizebox{\linewidth}{!}{%
\begin{tikzpicture}[x=1pt,y=1pt,font=\scriptsize,
  badge/.style={rounded corners=1.2pt,inner sep=1.2pt,text=white,font=\fontsize{5.2}{6}\selectfont\bfseries,anchor=south}]
\def\tw{42}\def\th{56}\def\tg{2}\def\rg{3.5}\def\xo{13}
\def\tile##1##2##3##4{%
  \pgfmathsetmacro\tx{\xo+(##1-1)*(\tw+\tg)}
  \begin{scope}
    \clip[rounded corners=1.6pt] (\tx,##2) rectangle ++(\tw,\th);
    \node[anchor=south west,inner sep=0pt] at (\tx,##2) {\includegraphics[width=\tw pt,height=\th pt]{##3}};
  \end{scope}
  \draw[rounded corners=1.6pt,##4] (\tx,##2) rectangle ++(\tw,\th);}
\pgfmathsetmacro\yv{2*(\th+\rg)}
\pgfmathsetmacro\yb{\th+\rg}
\pgfmathsetmacro\ya{\yv+\th+4}
\draw[black!35,line width=0.4pt,-{Latex[length=3pt,width=2.4pt]}] (\xo,\ya) -- (\xo+5*\tw+4*\tg+2,\ya);
\foreach \c/\t in {#2}{
  \pgfmathsetmacro\cx{\xo+(\c-1)*(\tw+\tg)+\tw/2}
  \draw[black!35,line width=0.4pt] (\cx,\ya-1.3) -- (\cx,\ya+1.3);
  \node[anchor=south,inner sep=1.2pt,text=black!70,font=\fontsize{5.6}{6.5}\selectfont] at (\cx,\ya+1.2) {\t\,s};}
\foreach \c in {1,...,5}{
  \tile{\c}{\yv}{#1v\c.jpg}{draw=black!25,line width=0.3pt}
  \tile{\c}{0}{#1o\c.jpg}{draw=black!18,line width=0.3pt}}
\foreach \c in {1,...,4}{\tile{\c}{\yb}{#1b\c.jpg}{draw=black!18,line width=0.3pt}}
\tile{5}{\yb}{#1b5.jpg}{draw=tsFall,line width=0.9pt}
\draw[rounded corners=1.6pt,draw=tsOk,line width=0.9pt] (\xo+4*\tw+4*\tg,0) rectangle ++(\tw,\th);
\node[badge,fill=tsFall] at (\xo+4*\tw+4*\tg+\tw/2,\yb+2.2) {\ding{55}\,fell at #3\,s};
\node[badge,fill=tsOk] at (\xo+4*\tw+4*\tg+\tw/2,2.2) {\ding{51}\,clip executed};
\node[rotate=90,align=center,font=\fontsize{6.2}{6.8}\selectfont,text=black!80] at (\xo/2-0.5,\yv+\th/2)
  {\textbf{Input video}\\[-0.2pt]+ our mesh};
\node[rotate=90,align=center,font=\fontsize{6.2}{6.8}\selectfont,text=tsBase] at (\xo/2-0.5,\yb+\th/2)
  {\textbf{GENMO}\\[-0.2pt]$\rightarrow$ robot};
\node[rotate=90,align=center,font=\fontsize{6.2}{6.8}\selectfont,text=tsOurs] at (\xo/2-0.5,\th/2)
  {\textbf{\method}\\[-0.2pt]robot mode};
\end{tikzpicture}}}
\begin{minipage}[t]{0.485\textwidth}\centering
\suppcase{figures/supp_cases/dance_}{1/0.5,2/2.0,3/3.5,4/5.0,5/7.2}{6.2}\\[1pt]
{\small (a) EMDB-1 P5\_42, dancing (0--10\,s)}
\end{minipage}\hfill
\begin{minipage}[t]{0.485\textwidth}\centering
\suppcase{figures/supp_cases/cross_}{1/1.0,2/3.0,3/5.0,4/7.0,5/9.3}{8.3}\\[1pt]
{\small (b) 3DPW downtown\_crossStreets\_00, crossing a street (0--10\,s)}
\end{minipage}\\[7pt]
\begin{minipage}[t]{0.485\textwidth}\centering
\suppcase{figures/supp_cases/rect_}{1/0.5,2/2.0,3/3.5,4/5.0,5/7.3}{6.3}\\[1pt]
{\small (c) EMDB-2 P9\_79, walking a rectangle (0--10\,s)}
\end{minipage}\hfill
\begin{minipage}[t]{0.485\textwidth}\centering
\suppcase{figures/supp_cases/park_}{1/0.5,2/2.0,3/3.5,4/5.0,5/7.3}{6.3}\\[1pt]
{\small (d) EMDB-2 P7\_61, walking in a park (20--30\,s)}
\end{minipage}


==> latexmkrc <==
# Build: latexmk -pdf main.tex   (also used by LaTeX Workshop's latexmk recipe)
# After every successful pdflatex run, main.pdf is split into
#   main_paper.pdf : main text + references (pages 1..\mainlastpage)
#   main_supp.pdf  : supplementary material (remaining pages)
# \mainlastpage is written to main.aux by main.tex right before the supplement.
# Splitting needs pdfinfo/pdfseparate/pdfunite (poppler-utils); if they are
# missing the split is skipped and the build itself is unaffected.

use File::Temp qw(tempdir);

$pdf_mode = 1;
$pdflatex = 'internal pdflatex_and_split %O %S';

sub pdflatex_and_split {
    my $ret = system('pdflatex', @_);
    return $ret if $ret != 0;
    my ($src) = grep { /\.tex$/ } @_;
    return 0 unless defined $src;
    (my $base = $src) =~ s{^.*/}{};
    $base =~ s{\.tex$}{};
    my $odir = $out_dir ne '' ? $out_dir : '.';
    my $adir = $aux_dir ne '' ? $aux_dir : $odir;
    split_main_supp("$odir/$base.pdf", "$adir/$base.aux", $odir);
    return 0;
}

sub split_main_supp {
    my ($pdf, $aux, $odir) = @_;
    return unless -e $pdf && -e $aux;
    open(my $fh, '<', $aux) or return;
    my $last;
    while (<$fh>) { $last = $1 if /\\gdef\s*\\mainlastpage\s*\{(\d+)\}/; }
    close $fh;
    return unless $last;
    my ($total) = (`pdfinfo "$pdf" 2>/dev/null` =~ /^Pages:\s+(\d+)/m);
    return unless $total && $total > $last;
    my $tmp = tempdir(CLEANUP => 1);
    return if system('pdfseparate', $pdf, "$tmp/p-%d.pdf") != 0;
    system('pdfunite', (map { "$tmp/p-$_.pdf" } 1 .. $last), "$odir/main_paper.pdf");
    system('pdfunite', (map { "$tmp/p-$_.pdf" } $last + 1 .. $total), "$odir/main_supp.pdf");
    print "latexmkrc: main_paper.pdf = pages 1-$last, main_supp.pdf = pages ", $last + 1, "-$total\n";
}


==> tables/components_steps.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{2.6pt}
\footnotesize
\renewcommand{\arraystretch}{0.9}
\caption{\textbf{Task branches and alignment over training:} control (C) \vs \method (E). MAE: set-point error ($^\circ$, training stream); errors in mm. Bold: lower.}
\label{tab:components_steps}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l cc cc cc cc cc}
\toprule
 & \multicolumn{2}{c}{MAE} & \multicolumn{2}{c}{3DPW MPJPE} & \multicolumn{2}{c}{RICH MPJPE} & \multicolumn{2}{c}{EMDB-1 MPJPE} & \multicolumn{2}{c}{EMDB-2 W} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}
Step & C & E & C & E & C & E & C & E & C & E \\
\midrule
30k & 8.4 & \best{6.3} & 56.4 & \best{56.3} & \best{65.0} & 65.5 & \best{63.8} & 64.4 & 369.3 & \best{346.4} \\
40k & 7.9 & \best{5.8} & \best{53.7} & 54.3 & \best{67.0} & 67.6 & \best{64.8} & 66.1 & 346.7 & \best{338.9} \\
50k & 7.4 & \best{5.5} & 54.8 & \best{53.7} & 65.9 & 65.9 & 64.8 & \best{64.7} & 382.1 & \best{330.4} \\
60k & 7.1 & \best{5.2} & \best{54.0} & 54.6 & 65.3 & \best{64.7} & \best{64.0} & 65.0 & 366.3 & \best{302.2} \\
70k & 6.8 & \best{5.1} & \best{55.0} & 55.1 & \best{65.9} & 66.0 & \best{65.2} & 65.3 & 346.7 & \best{309.0} \\
80k & 6.5 & \best{4.8} & 54.9 & \best{54.8} & 66.1 & \best{65.3} & \best{65.0} & 65.2 & 325.5 & \best{295.9} \\
110k & 6.1 & \best{4.5} & \best{54.4} & 54.8 & 66.4 & \best{65.1} & 65.5 & \best{64.9} & 318.8 & \best{282.6} \\
\bottomrule
\end{tabular}}
\end{table}


==> tables/corr.tex <==
\begin{table}[t]
\centering
\footnotesize\setlength{\tabcolsep}{4pt}
\caption{\textbf{Kinematic error \vs robot failure:} Spearman correlation of per-video human metrics with fall rate on GT-feasible segments (\corrPairs\ method--video pairs, EMDB and RICH).}
\label{tab:corr}
\resizebox{\linewidth}{!}{%
\begin{tabular}{cccccc}
\toprule
PA-MPJPE & MPJPE & W-MPJPE$_{100}$ & RTE & Jitter & Foot sliding \\
\midrule
$-0.02$ & $+0.05$ & $+0.32$ & $-0.04$ & $+0.22$ & $+0.22$ \\
\bottomrule
\end{tabular}}
\vspace{-1em}
\end{table}


==> tables/early10k.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{1.5pt}
\footnotesize
\renewcommand{\arraystretch}{0.9}
\caption{\textbf{Early checkpoints} (10k and 20k steps) of the ablation runs and of the sweep runs whose training stopped before 50k steps, all with the recipe of \method\ and evaluated as \method; every checkpoint that a run reached is listed. The alignment ramps up between 5k and 15k steps. Errors in mm.}
\label{tab:early10k}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ll ccc c cc cc cc cc}
\toprule
 & & & & & MAE & \multicolumn{2}{c}{3DPW} & \multicolumn{2}{c}{RICH} & \multicolumn{2}{c}{EMDB-1} & \multicolumn{2}{c}{EMDB-2} \\
\cmidrule(lr){7-8}\cmidrule(lr){9-10}\cmidrule(lr){11-12}\cmidrule(lr){13-14}
Step & Run & $\lambda_{\text{align}}$ & stride & seed & ($^\circ$) & PA & MPJPE & PA & MPJPE & PA & MPJPE & WA & W \\
\midrule
10k & Control & -- & -- & 42 & 11.18 & 38.8 & 59.9 & 44.7 & 69.5 & 44.8 & 69.2 & 157.8 & 393.5 \\
10k & w/o alignment & 0 & -- & 42 & 8.90 & 37.8 & 58.2 & 42.3 & 66.0 & 42.7 & 66.8 & 148.0 & 370.8 \\
10k & actions detached & 0 & -- & 42 & 8.97 & 38.6 & 60.1 & 42.6 & 65.6 & 43.1 & 66.3 & 142.4 & 357.4 \\
\rowcolor{red!6}10k & \method & 0.5 & 8 & 42 & 8.90 & 38.0 & 58.8 & 42.6 & 65.4 & 43.2 & 66.2 & 146.3 & 368.5 \\
10k & \method recipe & 0.5 & 8 & 43 & 8.49 & 37.6 & 59.0 & 42.3 & 65.6 & 43.2 & 65.3 & 142.0 & 349.7 \\
10k & \method recipe & 2 & 8 & 42 & 8.90 & 37.9 & 58.1 & 42.3 & 65.8 & 42.9 & 66.8 & 144.6 & 361.6 \\
10k & \method recipe & 0.5 & 2 & 42 & 8.90 & 38.2 & 59.2 & 42.4 & 65.4 & 43.2 & 67.1 & 151.6 & 384.9 \\
\midrule
20k & Control & -- & -- & 42 & 9.25 & 36.2 & 57.1 & 41.0 & 63.6 & 42.3 & 65.7 & 143.1 & 369.4 \\
20k & w/o alignment & 0 & -- & 42 & 7.13 & 36.3 & 59.0 & 40.1 & 63.0 & 42.2 & 65.4 & 143.1 & 377.3 \\
20k & actions detached & 0 & -- & 42 & 7.25 & 35.6 & 57.5 & 39.9 & 62.6 & 41.9 & 64.4 & 141.5 & 373.6 \\
\rowcolor{red!6}20k & \method & 0.5 & 8 & 42 & 7.13 & 36.0 & 58.5 & 39.7 & 63.2 & 42.0 & 65.2 & 141.5 & 376.9 \\
20k & \method recipe & 0.5 & 8 & 43 & 6.87 & 36.1 & 56.7 & 41.0 & 67.5 & 42.3 & 66.3 & 135.0 & 344.3 \\
20k & \method recipe & 2 & 8 & 42 & 7.13 & 36.2 & 59.9 & 40.5 & 64.0 & 42.1 & 64.7 & 146.2 & 388.7 \\
\bottomrule
\end{tabular}}
\vspace{-1em}
\end{table}


==> tables/human_unified.tex <==
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{2.2pt}
\scriptsize
\caption{\textbf{Human metrics of the motions we generate} on the 270 test videos (FlowHMR without RICH, \cref{sec:supp_baselines}; \cref{tab:robot} executes those of its \nVidBench\ videos), produced without test-time augmentation and scored with the official GENMO/GVHMR code (3DPW: 14 joints, others 24; DuoMo on its own vertices; \cref{sec:supp_baselines}).}
\label{tab:unified}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l cccc cccc cccc ccccc ccccc}
\toprule
 & \multicolumn{4}{c}{3DPW} & \multicolumn{4}{c}{EMDB-1} & \multicolumn{4}{c}{RICH (camera)} & \multicolumn{5}{c}{EMDB-2 (world)} & \multicolumn{5}{c}{RICH (world)} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}\cmidrule(lr){14-18}\cmidrule(lr){19-23}
Method & PA & MPJPE & PVE & Acc & PA & MPJPE & PVE & Acc & PA & MPJPE & PVE & Acc & WA & W & RTE & Jit. & FS & WA & W & RTE & Jit. & FS \\
\midrule
WHAM~\cite{shin2024wham}$^\dagger$ & 36.8 & 58.2 & 69.3 & 7.1 & 48.9 & 77.9 & 91.5 & 6.1 & 46.6 & 78.0 & 87.3 & 5.7 & 135.1 & 341.6 & 3.8 & 25.4 & 5.6 & 116.0 & 196.1 & 4.5 & 21.0 & 4.0 \\
GVHMR~\cite{shen2024gvhmr} & 37.0 & \second{56.5} & \second{68.6} & 5.2 & 43.8 & 73.9 & 85.4 & 4.0 & 42.1 & 67.8 & 75.6 & \second{4.2} & 111.1 & 274.7 & 2.0 & 16.7 & \second{3.5} & \second{80.9} & \second{129.4} & 2.4 & \second{12.8} & \best{3.0} \\
TRAM~\cite{wang2024tram}$^\dagger$ & \second{36.1} & 58.8 & 69.1 & 6.0 & 46.5 & 75.9 & 89.0 & 5.3 & 44.5 & 72.2 & 80.4 & 5.0 & \second{76.2} & \second{214.1} & \second{1.4} & 19.2 & 11.3 & 105.3 & 167.2 & \second{2.4} & 15.7 & 12.4 \\
DuoMo~\cite{wang2026duomo}$^\dagger$ & 36.3 & 57.7 & 69.5 & 7.1 & \best{41.3} & \second{66.8} & \second{77.9} & 6.3 & \best{37.9} & \best{55.3} & \best{62.8} & 5.4 & \best{66.8} & \best{166.6} & \best{1.2} & \second{9.4} & 3.9 & \best{55.4} & \best{82.1} & \best{1.3} & \best{6.2} & \second{3.2} \\
GENMO~\cite{li2025genmo} & 37.6 & 58.5 & 71.1 & 5.3 & 44.8 & 76.4 & 88.4 & 4.2 & 43.4 & 71.2 & 80.2 & 4.4 & 125.2 & 311.5 & 2.3 & 20.5 & 4.8 & 88.0 & 141.2 & 2.6 & 15.5 & 3.4 \\
FlowHMR~\cite{wang2026flowhmr} & 42.8 & 72.9 & 85.7 & \best{4.8} & 49.4 & 92.5 & 105.2 & \best{3.1} & -- & -- & -- & -- & 107.3 & 273.6 & 2.4 & \best{5.4} & \best{2.9} & -- & -- & -- & -- & -- \\
\rowcolor{red!6}\method & \best{35.0} & \best{54.9} & \best{66.2} & \second{4.9} & \second{42.3} & \best{66.3} & \best{77.9} & \second{3.3} & \second{38.7} & \second{65.9} & \second{73.8} & \best{4.0} & 129.8 & 334.5 & 3.0 & 19.9 & 7.8 & 93.1 & 153.4 & 2.8 & 15.0 & 4.1 \\
\bottomrule
\end{tabular}}
\end{table*}


==> tables/numbers_ablation_modules.tex <==
% auto-generated by figures/plot_figures.py from figures/data/ablation_modules.csv -- do not edit
\makeatletter
\newcommand{\amPending}{\textcolor{red}{[?]}}
\newcommand{\am@get}[1]{\@ifundefined{am@#1}{\amPending}{\@nameuse{am@#1}}}
\newcommand{\amM}[2]{\am@get{M@#1@#2}}
\newcommand{\amSD}[2]{\am@get{SD@#1@#2}}
\newcommand{\amP}[2]{\am@get{P@#1@#2}}
\newcommand{\amD}[2]{\am@get{D@#1@#2}}
\newcommand{\amG}[2]{\am@get{G@#1@#2}}
\newcommand{\amSh}[2]{\am@get{Sh@#1@#2}}
\@namedef{am@M@reg@succ_robot}{79.9}
\@namedef{am@P@reg@succ_robot}{$p{=}1.00$}
\@namedef{am@D@reg@succ_robot}{$-$6.1}
\@namedef{am@M@adapt@succ_robot}{81.7}
\@namedef{am@P@adapt@succ_robot}{$p{=}1.00$}
\@namedef{am@D@adapt@succ_robot}{$-$4.3}
\@namedef{am@M@temporal@succ_robot}{84.7}
\@namedef{am@P@temporal@succ_robot}{$p{=}1.00$}
\@namedef{am@D@temporal@succ_robot}{$-$1.3}
\@namedef{am@M@full@succ_robot}{86.0}
\@namedef{am@P@full@succ_robot}{$p{=}1.00$}
\@namedef{am@M@mlp_matched@succ_robot}{83.5}
\@namedef{am@P@mlp_matched@succ_robot}{$p{=}1.00$}
\@namedef{am@D@mlp_matched@succ_robot}{$-$2.5}
\@namedef{am@M@k1@succ_robot}{83.1}
\@namedef{am@P@k1@succ_robot}{$p{=}1.00$}
\@namedef{am@D@k1@succ_robot}{$-$2.9}
\@namedef{am@M@align_r2h@succ_robot}{84.9}
\@namedef{am@P@align_r2h@succ_robot}{$p{=}1.00$}
\@namedef{am@D@align_r2h@succ_robot}{$-$1.1}
\@namedef{am@M@align_h2r@succ_robot}{83.7}
\@namedef{am@P@align_h2r@succ_robot}{$p{=}1.00$}
\@namedef{am@D@align_h2r@succ_robot}{$-$2.3}
\@namedef{am@M@align_abs@succ_robot}{82.6}
\@namedef{am@P@align_abs@succ_robot}{$p{=}1.00$}
\@namedef{am@D@align_abs@succ_robot}{$-$3.4}
\@namedef{am@M@detach@succ_robot}{83.3}
\@namedef{am@P@detach@succ_robot}{$p{=}1.00$}
\@namedef{am@D@detach@succ_robot}{$-$2.7}
\@namedef{am@G@adapt@succ_robot}{$+$1.8}
\@namedef{am@Sh@adapt@succ_robot}{29}
\@namedef{am@G@temporal@succ_robot}{$+$3.0}
\@namedef{am@Sh@temporal@succ_robot}{49}
\@namedef{am@G@full@succ_robot}{$+$1.3}
\@namedef{am@Sh@full@succ_robot}{21}
\@namedef{am@M@reg@succ_human}{77.0}
\@namedef{am@P@reg@succ_human}{$p{=}1.00$}
\@namedef{am@D@reg@succ_human}{$-$4.0}
\@namedef{am@M@adapt@succ_human}{77.5}
\@namedef{am@P@adapt@succ_human}{$p{=}1.00$}
\@namedef{am@D@adapt@succ_human}{$-$3.5}
\@namedef{am@M@temporal@succ_human}{79.1}
\@namedef{am@P@temporal@succ_human}{$p{=}1.00$}
\@namedef{am@D@temporal@succ_human}{$-$1.9}
\@namedef{am@M@full@succ_human}{81.0}
\@namedef{am@P@full@succ_human}{$p{=}1.00$}
\@namedef{am@M@mlp_matched@succ_human}{78.8}
\@namedef{am@P@mlp_matched@succ_human}{$p{=}1.00$}
\@namedef{am@D@mlp_matched@succ_human}{$-$2.2}
\@namedef{am@M@k1@succ_human}{79.9}
\@namedef{am@P@k1@succ_human}{$p{=}1.00$}
\@namedef{am@D@k1@succ_human}{$-$1.1}
\@namedef{am@M@align_r2h@succ_human}{77.2}
\@namedef{am@P@align_r2h@succ_human}{$p{=}1.00$}
\@namedef{am@D@align_r2h@succ_human}{$-$3.8}
\@namedef{am@M@align_h2r@succ_human}{77.1}
\@namedef{am@P@align_h2r@succ_human}{$p{=}1.00$}
\@namedef{am@D@align_h2r@succ_human}{$-$3.9}
\@namedef{am@M@align_abs@succ_human}{75.5}
\@namedef{am@P@align_abs@succ_human}{$p{=}1.00$}
\@namedef{am@D@align_abs@succ_human}{$-$5.5}
\@namedef{am@M@detach@succ_human}{78.3}
\@namedef{am@P@detach@succ_human}{$p{=}1.00$}
\@namedef{am@D@detach@succ_human}{$-$2.7}
\@namedef{am@G@adapt@succ_human}{$+$0.5}
\@namedef{am@Sh@adapt@succ_human}{12}
\@namedef{am@G@temporal@succ_human}{$+$1.6}
\@namedef{am@Sh@temporal@succ_human}{40}
\@namedef{am@G@full@succ_human}{$+$1.9}
\@namedef{am@Sh@full@succ_human}{48}
\@namedef{am@M@reg@mae}{7.42}
\@namedef{am@P@reg@mae}{$p{=}0.10$}
\@namedef{am@D@reg@mae}{$+$1.93}
\@namedef{am@M@adapt@mae}{7.15}
\@namedef{am@P@adapt@mae}{$p{=}0.10$}
\@namedef{am@D@adapt@mae}{$+$1.66}
\@namedef{am@M@temporal@mae}{5.59}
\@namedef{am@P@temporal@mae}{$p{=}1.00$}
\@namedef{am@D@temporal@mae}{$+$0.10}
\@namedef{am@M@full@mae}{5.49}
\@namedef{am@P@full@mae}{$p{=}1.00$}
\@namedef{am@M@mlp_matched@mae}{7.02}
\@namedef{am@P@mlp_matched@mae}{$p{=}0.10$}
\@namedef{am@D@mlp_matched@mae}{$+$1.53}
\@namedef{am@M@k1@mae}{5.86}
\@namedef{am@P@k1@mae}{$p{=}0.10$}
\@namedef{am@D@k1@mae}{$+$0.37}
\@namedef{am@M@align_r2h@mae}{5.49}
\@namedef{am@P@align_r2h@mae}{$p{=}1.00$}
\@namedef{am@D@align_r2h@mae}{0.00}
\@namedef{am@M@align_h2r@mae}{5.49}
\@namedef{am@P@align_h2r@mae}{$p{=}1.00$}
\@namedef{am@D@align_h2r@mae}{0.00}
\@namedef{am@M@align_abs@mae}{5.95}
\@namedef{am@P@align_abs@mae}{$p{=}0.10$}
\@namedef{am@D@align_abs@mae}{$+$0.46}
\@namedef{am@M@detach@mae}{5.91}
\@namedef{am@P@detach@mae}{$p{=}0.10$}
\@namedef{am@D@detach@mae}{$+$0.42}
\@namedef{am@G@adapt@mae}{$-$0.27}
\@namedef{am@Sh@adapt@mae}{14}
\@namedef{am@G@temporal@mae}{$-$1.56}
\@namedef{am@Sh@temporal@mae}{81}
\@namedef{am@G@full@mae}{$-$0.10}
\@namedef{am@Sh@full@mae}{5}
\@namedef{am@M@reg@mpjpe_3dpw}{54.8}
\@namedef{am@P@reg@mpjpe_3dpw}{$p{=}1.00$}
\@namedef{am@D@reg@mpjpe_3dpw}{$+$1.1}
\@namedef{am@M@adapt@mpjpe_3dpw}{54.8}
\@namedef{am@P@adapt@mpjpe_3dpw}{$p{=}1.00$}
\@namedef{am@D@adapt@mpjpe_3dpw}{$+$1.1}
\@namedef{am@M@temporal@mpjpe_3dpw}{54.8}
\@namedef{am@P@temporal@mpjpe_3dpw}{$p{=}1.00$}
\@namedef{am@D@temporal@mpjpe_3dpw}{$+$1.1}
\@namedef{am@M@full@mpjpe_3dpw}{53.7}
\@namedef{am@P@full@mpjpe_3dpw}{$p{=}1.00$}
\@namedef{am@M@mlp_matched@mpjpe_3dpw}{53.9}
\@namedef{am@P@mlp_matched@mpjpe_3dpw}{$p{=}1.00$}
\@namedef{am@D@mlp_matched@mpjpe_3dpw}{$+$0.2}
\@namedef{am@M@k1@mpjpe_3dpw}{53.8}
\@namedef{am@P@k1@mpjpe_3dpw}{$p{=}1.00$}
\@namedef{am@D@k1@mpjpe_3dpw}{$+$0.1}
\@namedef{am@M@align_r2h@mpjpe_3dpw}{53.9}
\@namedef{am@P@align_r2h@mpjpe_3dpw}{$p{=}1.00$}
\@namedef{am@D@align_r2h@mpjpe_3dpw}{$+$0.2}
\@namedef{am@M@align_h2r@mpjpe_3dpw}{54.8}
\@namedef{am@P@align_h2r@mpjpe_3dpw}{$p{=}1.00$}
\@namedef{am@D@align_h2r@mpjpe_3dpw}{$+$1.1}
\@namedef{am@M@align_abs@mpjpe_3dpw}{55.6}
\@namedef{am@P@align_abs@mpjpe_3dpw}{$p{=}0.10$}
\@namedef{am@D@align_abs@mpjpe_3dpw}{$+$1.9}
\@namedef{am@M@detach@mpjpe_3dpw}{54.4}
\@namedef{am@P@detach@mpjpe_3dpw}{$p{=}1.00$}
\@namedef{am@D@detach@mpjpe_3dpw}{$+$0.7}
\@namedef{am@G@adapt@mpjpe_3dpw}{0.0}
\@namedef{am@Sh@adapt@mpjpe_3dpw}{0}
\@namedef{am@G@temporal@mpjpe_3dpw}{0.0}
\@namedef{am@Sh@temporal@mpjpe_3dpw}{0}
\@namedef{am@G@full@mpjpe_3dpw}{$-$1.1}
\@namedef{am@Sh@full@mpjpe_3dpw}{100}
\@namedef{am@M@reg@mpjpe_emdb1}{65.8}
\@namedef{am@P@reg@mpjpe_emdb1}{$p{=}1.00$}
\@namedef{am@D@reg@mpjpe_emdb1}{$+$1.1}
\@namedef{am@M@adapt@mpjpe_emdb1}{65.0}
\@namedef{am@P@adapt@mpjpe_emdb1}{$p{=}1.00$}
\@namedef{am@D@adapt@mpjpe_emdb1}{$+$0.3}
\@namedef{am@M@temporal@mpjpe_emdb1}{65.2}
\@namedef{am@P@temporal@mpjpe_emdb1}{$p{=}1.00$}
\@namedef{am@D@temporal@mpjpe_emdb1}{$+$0.5}
\@namedef{am@M@full@mpjpe_emdb1}{64.7}
\@namedef{am@P@full@mpjpe_emdb1}{$p{=}1.00$}
\@namedef{am@M@mlp_matched@mpjpe_emdb1}{64.6}
\@namedef{am@P@mlp_matched@mpjpe_emdb1}{$p{=}1.00$}
\@namedef{am@D@mlp_matched@mpjpe_emdb1}{$-$0.1}
\@namedef{am@M@k1@mpjpe_emdb1}{64.8}
\@namedef{am@P@k1@mpjpe_emdb1}{$p{=}1.00$}
\@namedef{am@D@k1@mpjpe_emdb1}{$+$0.1}
\@namedef{am@M@align_r2h@mpjpe_emdb1}{64.8}
\@namedef{am@P@align_r2h@mpjpe_emdb1}{$p{=}1.00$}
\@namedef{am@D@align_r2h@mpjpe_emdb1}{$+$0.1}
\@namedef{am@M@align_h2r@mpjpe_emdb1}{65.2}
\@namedef{am@P@align_h2r@mpjpe_emdb1}{$p{=}1.00$}
\@namedef{am@D@align_h2r@mpjpe_emdb1}{$+$0.5}
\@namedef{am@M@align_abs@mpjpe_emdb1}{65.9}
\@namedef{am@P@align_abs@mpjpe_emdb1}{$p{=}0.10$}
\@namedef{am@D@align_abs@mpjpe_emdb1}{$+$1.2}
\@namedef{am@M@detach@mpjpe_emdb1}{65.1}
\@namedef{am@P@detach@mpjpe_emdb1}{$p{=}1.00$}
\@namedef{am@D@detach@mpjpe_emdb1}{$+$0.4}
\@namedef{am@G@adapt@mpjpe_emdb1}{$-$0.8}
\@namedef{am@Sh@adapt@mpjpe_emdb1}{73}
\@namedef{am@G@temporal@mpjpe_emdb1}{$+$0.2}
\@namedef{am@Sh@temporal@mpjpe_emdb1}{$-$18}
\@namedef{am@G@full@mpjpe_emdb1}{$-$0.5}
\@namedef{am@Sh@full@mpjpe_emdb1}{45}
\@namedef{am@M@reg@wmpjpe_emdb2}{177.7}
\@namedef{am@P@reg@wmpjpe_emdb2}{$p{=}0.002$}
\@namedef{am@D@reg@wmpjpe_emdb2}{$+$1.0}
\@namedef{am@M@adapt@wmpjpe_emdb2}{178.0}
\@namedef{am@P@adapt@wmpjpe_emdb2}{$p{=}0.09$}
\@namedef{am@D@adapt@wmpjpe_emdb2}{$+$1.3}
\@namedef{am@M@temporal@wmpjpe_emdb2}{177.6}
\@namedef{am@P@temporal@wmpjpe_emdb2}{$p{=}0.14$}
\@namedef{am@D@temporal@wmpjpe_emdb2}{$+$0.9}
\@namedef{am@M@full@wmpjpe_emdb2}{176.7}
\@namedef{am@P@full@wmpjpe_emdb2}{$p{=}1.00$}
\@namedef{am@M@mlp_matched@wmpjpe_emdb2}{180.0}
\@namedef{am@P@mlp_matched@wmpjpe_emdb2}{$p{=}0.09$}
\@namedef{am@D@mlp_matched@wmpjpe_emdb2}{$+$3.3}
\@namedef{am@M@k1@wmpjpe_emdb2}{179.5}
\@namedef{am@P@k1@wmpjpe_emdb2}{$p{=}1.00$}
\@namedef{am@D@k1@wmpjpe_emdb2}{$+$2.8}
\@namedef{am@M@align_r2h@wmpjpe_emdb2}{178.2}
\@namedef{am@P@align_r2h@wmpjpe_emdb2}{$p{=}1.00$}
\@namedef{am@D@align_r2h@wmpjpe_emdb2}{$+$1.5}
\@namedef{am@M@align_h2r@wmpjpe_emdb2}{177.5}
\@namedef{am@P@align_h2r@wmpjpe_emdb2}{$p{=}1.00$}
\@namedef{am@D@align_h2r@wmpjpe_emdb2}{$+$0.8}
\@namedef{am@M@align_abs@wmpjpe_emdb2}{178.2}
\@namedef{am@P@align_abs@wmpjpe_emdb2}{$p{=}1.00$}
\@namedef{am@D@align_abs@wmpjpe_emdb2}{$+$1.5}
\@namedef{am@M@detach@wmpjpe_emdb2}{177.2}
\@namedef{am@P@detach@wmpjpe_emdb2}{$p{=}1.00$}
\@namedef{am@D@detach@wmpjpe_emdb2}{$+$0.5}
\@namedef{am@G@adapt@wmpjpe_emdb2}{$+$0.3}
\@namedef{am@Sh@adapt@wmpjpe_emdb2}{$-$30}
\@namedef{am@G@temporal@wmpjpe_emdb2}{$-$0.4}
\@namedef{am@Sh@temporal@wmpjpe_emdb2}{40}
\@namedef{am@G@full@wmpjpe_emdb2}{$-$0.9}
\@namedef{am@Sh@full@wmpjpe_emdb2}{90}
\makeatother


==> tables/sweep.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{1.6pt}
\footnotesize
\renewcommand{\arraystretch}{0.9}
\caption{\textbf{Alignment hyperparameters and seeds.} Every run of the sweep over the alignment weight $\lambda_{\text{align}}$ and the alignment frame stride and of the repeated seeds, all with the recipe of \method\ at 50k steps and evaluated as \method; none of them was selected or discarded. Errors in mm, success in \%.}
\label{tab:sweep}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l ccc c cc cc cc cc cc}
\toprule
 & & & & MAE & \multicolumn{2}{c}{3DPW} & \multicolumn{2}{c}{RICH} & \multicolumn{2}{c}{EMDB-1} & \multicolumn{2}{c}{EMDB-2} & \multicolumn{2}{c}{Succ.} \\
\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}\cmidrule(lr){14-15}
Run & $\lambda_{\text{align}}$ & stride & seed & ($^\circ$) & PA & MPJPE & PA & MPJPE & PA & MPJPE & WA & W & human & robot \\
\midrule
w/o alignment & 0 & -- & 42 & 5.49 & 34.8 & 54.8 & 38.5 & 66.3 & 40.9 & 65.2 & 127.5 & 323.4 & 76.1 & 85.8 \\
w/o alignment & 0 & -- & 43 & XX & XX & XX & XX & XX & XX & XX & XX & XX & XX & XX \\
actions detached & 0 & -- & 42 & 5.61 & 34.5 & 54.4 & 38.4 & 66.0 & 40.7 & 64.1 & 128.7 & 330.6 & 76.3 & 85.3 \\
actions detached & 0 & -- & 43 & XX & XX & XX & XX & XX & XX & XX & XX & XX & XX & XX \\
\rowcolor{red!6}\method & 0.5 & 8 & 42 & 5.49 & 34.3 & 53.7 & 38.7 & 65.9 & 40.8 & 64.7 & 128.9 & 330.4 & 77.0 & 86.0 \\
\method recipe & 0.5 & 8 & 43 & XX & XX & XX & XX & XX & XX & XX & XX & XX & XX & XX \\
\method recipe & 1 & 8 & 42 & XX & XX & XX & XX & XX & XX & XX & XX & XX & XX & XX \\
\method recipe & 2 & 8 & 42 & XX & XX & XX & XX & XX & XX & XX & XX & XX & XX & XX \\
\method recipe & 0.5 & 2 & 42 & XX & XX & XX & XX & XX & XX & XX & XX & XX & XX & XX \\
\bottomrule
\end{tabular}}
\vspace{-1em}
\end{table}


==> tables/tta.tex <==
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{3.2pt}
\footnotesize
\caption{\textbf{Test-time calibration} (all test sequences, no FlipEval). GENMO's protocol uses $f{=}\max(w,h)$ on EMDB and the dataset intrinsics on 3DPW and RICH. Decoding with the dataset intrinsics changes only the camera-frame translation, none of these metrics. Shape: per-sequence median PromptHMR betas replace ours or set only the height ($\beta_0$); the root is rescaled to keep the projection.}
\label{tab:tta}
\begin{tabular}{l cc ccc cccc ccc}
\toprule
 & \multicolumn{2}{c}{3DPW} & \multicolumn{3}{c}{EMDB-1} & \multicolumn{4}{c}{RICH} & \multicolumn{3}{c}{EMDB-2 (world)} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-6}\cmidrule(lr){7-10}\cmidrule(lr){11-13}
Variant & PA & MPJPE & PA & MPJPE & PVE & PA & MPJPE & PVE & WA & WA & W & FS \\
\midrule
\method, no calibration ($f{=}\max(w,h)$ on EMDB) & 35.0 & \best{54.9} & 42.3 & \best{66.3} & \best{77.9} & 38.7 & 65.9 & 73.8 & 93.1 & \best{129.8} & \best{334.5} & \best{7.8} \\
dataset intrinsics as network input (EMDB) & 35.0 & \best{54.9} & \best{42.1} & 66.6 & 78.4 & 38.7 & 65.9 & 73.8 & 93.1 & 139.1 & 363.5 & 9.0 \\
decoding with dataset intrinsics + PromptHMR shape & \best{34.8} & 55.9 & 43.0 & 74.7 & 86.0 & \best{38.1} & \best{58.1} & \best{66.8} & \best{92.7} & 131.5 & 339.0 & 8.1 \\
decoding with dataset intrinsics + PromptHMR height & 35.0 & 55.8 & 42.4 & 71.2 & 83.0 & 38.7 & 59.5 & 68.0 & 93.0 & 130.1 & 335.7 & 8.1 \\
\bottomrule
\end{tabular}
\end{table*}

